Addressing Outstanding Problems in the Physics of Massive Stars with the Line Emission Mapper X-ray Probe

We present some of the salient aspects of the scientific motivation for high resolution soft X-ray spectroscopy of early-type stars with the Line Emission Mapper X-ray Probe. The major strength of {\it LEM} for hot star physics is its large effective area, aided by the inherent energy resolution of its microcalorimeter that readily achieves resolving powers of 1000 and obviates the need for relatively inefficient dispersive optical elements. This increased sensitivity enables much fainter and more distant high mass stars to be observed than are accessible with present-day facilities, greatly increasing the pool of potential targets. For brighter sources, the sensitivity opens up time domain studies, wherein sufficient signal can be garnered in short order and exposure times, probing source variations on ks timescales. We argue that these capabilities of {\it LEM} will yield breakthroughs in all types of hot star systems, from understanding single OB and WR star winds and how they vary with metallicity, to probing the shocks of colliding wind systems and the magnetically channeled winds of magnetic OB stars. {\it LEM} will also study the energetics of WR star bubbles and feedback from their powerful pre-SN stellar winds.

==> Exo_refs-archive.tex <==
{\small

\noindent %\bibitem[Airapetian et al.(2016)]{Airapetian et al.(2016)} 
Airapetian, V.~S., Glocer, A., Gronoff, G., H{\'e}brard, E., \& Danchi, W.\ 2016, Nature Geoscience, 9, 452\\

\noindent %\bibitem[Bhardwaj et al.(2007)]{Bhardwaj et al.(2007)}
 Bhardwaj, A., et al.\ 2007, Planetary and Space Science, 55, 1135\\

\noindent %\bibitem[Cravens, Robertson, \& Snowden(2001)]{Cravens et al.(2001)} 
Cravens, T.~E., Robertson, I.~P., \& Snowden, S.~L.\ 2001, \jgr, 106, 24883 \\

\noindent %\bibitem[Cuntz, Saar, \& Musielak(2000)]{Cuntz et al.(2000)} 
Cuntz, M., Saar, S.~H., \& Musielak, Z.~E.\ 2000, \apjl, 533, L151\\

\noindent %\bibitem[Dong et al.(2018)]{Dong et al.(2018)} D
Dong, C.~F., Jin, M., Lingam, M., Airapetian, V. S., Ma, Y. J., van der Holst, B.\ 2018, Proc. Natl. Acad. Sci., 115, 260\\

\noindent %\bibitem[Ehrenreich et al.(2015)]{Ehrenreich et al.(2015)} 
Ehrenreich, D., et al.\ 2015, \nat, 522, 459 \\

\noindent %\bibitem[Erkaev et al.(2007)]{Erkaev et al.(2007)}
 Erkaev, N.~V., Kulikov, Y.~N., Lammer, H., Selsis, F., Langmayr, D., Jaritz, G.~F., \& Biernat, H.~K.\ 2007, \aap, 472, 329 \\

\noindent%\bibitem[Fossati et al.(2010)]{Fossati et al.(2010)} 
Fossati, L., et al.\ 2010, \apjl, 714, L222 \\

\noindent%\bibitem[Fulton \& Petigura(2018)]{Fulton et al.(2018)} 
Fulton, B.~J., \& Petigura, E.~A.\ 2018, \aj, 156, 264\\

\noindent%\bibitem[Gillon et al.(2017)]{Gillon et al.(2017)} 
Gillon, M., et al.\ 2017, \nat, 542, 456 \\

\noindent%\bibitem[Guedel(2007)]{Guedel(2007)}
 G{\"u}del, M.\ 2007, Living Reviews in Solar Physics, 4, 3 \\

\noindent%\bibitem[Iro \& Deming(2010)]{Iro et al.(2010)} 
Iro, N., \& Deming, L.~D.\ 2010, \apj, 712, 218 \\

\noindent%\bibitem[Kashyap, Drake, \& Saar(2008)]{Kashyap et al.(2008)} 
Kashyap, V.~L., Drake, J.~J., \& Saar, S.~H.\ 2008, \apj, 687, 1339\\

\noindent%\bibitem[Kulow et al.(2014)]{Kulow et al.(2014)} 
Kulow, J.~R., France, K., Linsky, J., \& Loyd, R.~O.~P.\ 2014, \apj, 786, 132 \\

\noindent%\bibitem[Lalitha, Schmitt, \& Dash(2018)]{Lalitha et al.(2018)} 
Lalitha, S., Schmitt, J.~H.~M.~M., \& Dash, S.\ 2018, \mnras, 477, 808 \\

\noindent%\bibitem[Lammer et al.(2003)]{Lammer et al.(2003)} 
Lammer, H., Selsis, F., Ribas, I., Guinan, E.~F., Bauer, S.~J., \& Weiss, W.~W.\ 2003, \apjl, 598, L121 \\

\noindent%\bibitem[Lanza(2009)]{Lanza(2009)} 
Lanza, A.~F.\ 2009, \aap, 505, 339 \\

\noindent%\bibitem[Lanza(2012)]{Lanza(2012)}
 Lanza, A.~F.\ 2012, \aap, 544, A23 \\

\noindent%\bibitem[Lavie et al.(2017)]{Lavie et al.(2017)} 
Lavie, B., et al.\ 2017,  \aap, 605, L7 \\

\noindent%\bibitem[Lecavelier des Etangs et al.(2012)]{Lecavelier des Etangs et al.(2012)}
 Lecavelier des Etangs, A., et al.\ 2012, \aap, 543, L4 \\

\noindent%\bibitem[Lingam et al.(2018)]{Lingam et al.(2018)} 
Lingam, M., Dong, C. F., Fang, X. H., Jakosky, B. M., Loeb, A.\ 2018, \apj, 853, 10 \\

\noindent%\bibitem[Linsky et al.(2010)]{Linsky et al.(2010)}
 Linsky, J.~L., Yang, H., France, K., Froning, C.~S., Green, J.~C., Stocke, J.~T., \& Osterman, S.~N.\ 2010, \apj, 717, 1291 \\

\noindent%\bibitem[Llama \& Shkolnik(2015)]{Llama et al.(2015)}
 Llama, J., \& Shkolnik, E.~L.\ 2015, \apj, 802, 41 \\
 
\noindent%\bibitem[Lopez \& Fortney(2013)]{Lopez et al.(2013)}
Lopez, E.~D., \& Fortney, J.~J.\ 2013, \apj, 776, 2 \\

\noindent%\bibitem[Maggio et al.(2015)]{Maggio et al.(2015)} 
Maggio, A., et al.\ 2015, \apjl, 811, L2 \\

\noindent%\bibitem[Miller et al.(2015)]{Miller et al.(2015)} 
Miller, B.~P., Gallo, E., Wright, J.~T., \& Pearson, E.~G.\ 2015, \apj, 799, 163 \\

\noindent%\bibitem[Murray-Clay, Chiang, \& Murray(2009)]{Murray-Clay et al.(2009)} 
Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 \\

\noindent%\bibitem[Owen \& Wu(2017)]{Owen et al.(2017)} 
Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 \\

\noindent%\bibitem[Owen \& Lai(2018)]{Owen et al.(2018)} 
Owen, J.~E., \& Lai, D.\ 2018, \mnras, 479, 5012 \\

\noindent%\bibitem[Penz, Micela,  \& Lammer(2008)]{Penz et al.(2008)} 
Penz, T., Micela, G., \& Lammer, H.\ 2008, \aap, 477, 309 \\

\noindent%\bibitem[Pillitteri et al.(2011)]{Pillitteri et al.(2011)} 
Pillitteri, I., G{\"u}nther, H.~M., Wolk, S.~J., Kashyap, V.~L., \& Cohen, O.\ 2011, \apjl, 741, L18 \\

\noindent%\bibitem[Pillitteri et al.(2014)]{Pillitteri et al.(2014)} 
Pillitteri, I., Wolk, S.~J., Lopez-Santiago, J., G{\"u}nther, H.~M., Sciortino, S., Cohen, O., Kashyap, V., \& Drake, J.~J.\ 2014, \apj, 785, 145 \\

\noindent%\bibitem[Poppenhaeger, Schmitt, \& Wolk(2013)]{Poppenhaeger et al.(2013)} 
Poppenhaeger, K., Schmitt, J.~H.~M.~M., \& Wolk, S.~J.\ 2013, \apj, 773, 62 \\

\noindent%\bibitem[Poppenhaeger \& Wolk(2014)]{Poppenhaeger et al.(2014)} 
Poppenhaeger, K., \& Wolk, S.~J.\ 2014, \aap, 565, L1 \\

\noindent%\bibitem[Sanz-Forcada et al.(2010)]{Sanz-Forcada et al.(2010)} 
Sanz-Forcada, J., Ribas, I., Micela, G., Pollock, A.~M.~T., Garc{\'{\i}}a-{\'A}lvarez, D., Solano, E., \& Eiroa, C.\ 2010, \aap, 511, L8 \\

\noindent%\bibitem[Tian et al.(2005)]{Tian et al.(2005)}
 Tian, F., Toon, O.~B., Pavlov, A.~A., \& De Sterck, H.\ 2005, Science, 308, 1014 \\

\noindent%\bibitem[Vidal-Madjar et al.(2003)]{Vidal-Madjar et al.(2003)} 
Vidal-Madjar, A., Lecavelier des Etangs, A., D{\'e}sert, J.-M., Ballester, G.~E., Ferlet, R., H{\'e}brard, G., \& Mayor, M.\ 2003, \nat, 422, 143\\

\noindent%\bibitem[Wood et al.(2018)]{Wood et al.(2018)} 
Wood, B.~E., Laming, J.~M., Warren, H.~P., \& Poppenhaeger, K.\ 2018, \apj, 862, 66 \\

\noindent%\bibitem[Yelle(2004)]{Yelle(2004)} 
Yelle, R.~V.\ 2004, Icarus, 170, 167 \\
}
%\end{bibliograpghy)

==> Exo_refs.tex <==

\bibitem[Airapetian et al.(2016)]{Airapetian et al.(2016)} Airapetian, V.~S., Glocer, A., Gronoff, G., H{\'e}brard, E., \& Danchi, W.\ 2016, Nature Geoscience, 9, 452

\bibitem[Bhardwaj et al.(2007)]{Bhardwaj et al.(2007)} Bhardwaj, A., et 
al.\ 2007, Planetary and Space Science, 55, 1135

\bibitem[Cravens, Robertson, \& Snowden(2001)]{Cravens et al.(2001)} Cravens, T.~E., Robertson, I.~P., \& Snowden, S.~L.\ 2001, \jgr, 106, 24883 

\bibitem[Cuntz, Saar, \& Musielak(2000)]{Cuntz et al.(2000)} Cuntz, M., Saar, S.~H., \& Musielak, Z.~E.\ 2000, \apjl, 533, L151

\bibitem[Dong et al.(2018)]{Dong et al.(2018)} Dong, C.~F., Jin, M., Lingam, M., Airapetian, V. S., Ma, Y. J., van der Holst, B.\ 2018, Proc. Natl. Acad. Sci., 115, 260

\bibitem[Ehrenreich et al.(2015)]{Ehrenreich et al.(2015)} Ehrenreich, D., 
et al.\ 2015, \nat, 522, 459 

\bibitem[Erkaev et al.(2007)]{Erkaev et al.(2007)} Erkaev, N.~V., Kulikov, Y.~N., Lammer, H., Selsis, F., Langmayr, D., Jaritz, G.~F., \& Biernat, H.~K.\ 2007, \aap, 472, 329 

\bibitem[Fossati et al.(2010)]{Fossati et al.(2010)} Fossati, L., et al.\ 2010, \apjl, 714, L222 

\bibitem[Fulton \& Petigura(2018)]{Fulton et al.(2018)} Fulton, B.~J., \& Petigura, E.~A.\ 2018, \aj, 156, 264

\bibitem[Gillon et al.(2017)]{Gillon et al.(2017)} Gillon, M., et al.\ 2017, \nat, 542, 456 

\bibitem[Guedel(2007)]{Guedel(2007)} G{\"u}del, M.\ 2007, Living Reviews in Solar Physics, 4, 3 

\bibitem[Iro \& Deming(2010)]{Iro et al.(2010)} Iro, N., \& Deming, L.~D.\ 2010, \apj, 712, 218 

\bibitem[Kashyap, Drake, \& Saar(2008)]{Kashyap et al.(2008)} Kashyap, V.~L., Drake, J.~J., \& Saar, S.~H.\ 2008, \apj, 687, 

\bibitem[Kulow et al.(2014)]{Kulow et al.(2014)} Kulow, J.~R., France, K., Linsky, J., \& Loyd, R.~O.~P.\ 2014, \apj, 786, 132 

\bibitem[Lalitha, Schmitt, \& Dash(2018)]{Lalitha et al.(2018)} Lalitha, S., Schmitt, J.~H.~M.~M., \& Dash, S.\ 2018, \mnras, 477, 808 

\bibitem[Lammer et al.(2003)]{Lammer et al.(2003)} Lammer, H., Selsis, F., Ribas, I., Guinan, E.~F., Bauer, S.~J., \& Weiss, W.~W.\ 2003, \apjl, 598, L121 

\bibitem[Lanza(2009)]{Lanza(2009)} Lanza, A.~F.\ 2009, \aap, 505, 339 

\bibitem[Lanza(2012)]{Lanza(2012)} Lanza, A.~F.\ 2012, \aap, 544, A23 

\bibitem[Lavie et al.(2017)]{Lavie et al.(2017)} Lavie, B., et al.\ 2017,  \aap, 605, L7 

\bibitem[Lecavelier des Etangs et al.(2012)]{Lecavelier des Etangs et al.(2012)} Lecavelier des Etangs, A., et al.\ 2012, \aap, 543, L4 

\bibitem[Lingam et al.(2018)]{Lingam et al.(2018)} Lingam, M., Dong, C. F., Fang, X. H., Jakosky, B. M., Loeb, A.\ 2018, \apj, 853, 10 

\bibitem[Linsky et al.(2010)]{Linsky et al.(2010)} Linsky, J.~L., Yang, H., France, K., Froning, C.~S., Green, J.~C., Stocke, J.~T., \& Osterman, S.~N.\ 2010, \apj, 717, 1291 

\bibitem[Llama \& Shkolnik(2015)]{Llama et al.(2015)} Llama, J., \& Shkolnik, E.~L.\ 2015, \apj, 802, 41 
\bibitem[Lopez \& Fortney(2013)]{Lopez et al.(2013)} Lopez, E.~D., \& Fortney, J.~J.\ 2013, \apj, 776, 2 

\bibitem[Maggio et al.(2015)]{Maggio et al.(2015)} Maggio, A., et al.\ 2015, \apjl, 811, L2 

\bibitem[Miller et al.(2015)]{Miller et al.(2015)} Miller, B.~P., Gallo, E., Wright, J.~T., \& Pearson, E.~G.\ 2015, \apj, 799, 163 

\bibitem[Murray-Clay, Chiang, \& Murray(2009)]{Murray-Clay et al.(2009)} Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 

\bibitem[Owen \& Wu(2017)]{Owen et al.(2017)} Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 

\bibitem[Owen \& Lai(2018)]{Owen et al.(2018)} Owen, J.~E., \& Lai, D.\ 2018, \mnras, 479, 5012 

\bibitem[Penz, Micela,  \& Lammer(2008)]{Penz et al.(2008)} Penz, T., Micela, G., \& Lammer, H.\ 2008, \aap, 477, 309 

\bibitem[Pillitteri et al.(2011)]{Pillitteri et al.(2011)} Pillitteri, I., G{\"u}nther, H.~M., Wolk, S.~J., Kashyap, V.~L., \& Cohen, O.\ 2011, \apjl, 741, L18 

\bibitem[Pillitteri et al.(2014)]{Pillitteri et al.(2014)} Pillitteri, I., Wolk, S.~J., Lopez-Santiago, J., G{\"u}nther, H.~M., Sciortino, S., Cohen, O., Kashyap, V., \& Drake, J.~J.\ 2014, \apj, 785, 145 

\bibitem[Poppenhaeger, Schmitt, \& Wolk(2013)]{Poppenhaeger et al.(2013)} Poppenhaeger, K., Schmitt, J.~H.~M.~M., \& Wolk, S.~J.\ 2013, \apj, 773, 62 

\bibitem[Poppenhaeger \& Wolk(2014)]{Poppenhaeger et al.(2014)} Poppenhaeger, K., \& Wolk, S.~J.\ 2014, \aap, 565, L1 

\bibitem[Sanz-Forcada et al.(2010)]{Sanz-Forcada et al.(2010)} Sanz-Forcada, J., Ribas, I., Micela, G., Pollock, A.~M.~T., Garc{\'{\i}}a-{\'A}lvarez, D., Solano, E., \& Eiroa, C.\ 2010, \aap, 511, L8 

\bibitem[Tian et al.(2005)]{Tian et al.(2005)} Tian, F., Toon, O.~B., Pavlov, A.~A., \& De Sterck, H.\ 2005, Science, 308, 1014 

\bibitem[Vidal-Madjar et al.(2003)]{Vidal-Madjar et al.(2003)} Vidal-Madjar, A., Lecavelier des Etangs, A., D{\'e}sert, J.-M., Ballester, G.~E., Ferlet, R., H{\'e}brard, G., \& Mayor, M.\ 2003, \nat, 422, 143

\bibitem[Wood et al.(2018)]{Wood et al.(2018)} Wood, B.~E., Laming, J.~M., Warren, H.~P., \& Poppenhaeger, K.\ 2018, \apj, 862, 66 

\bibitem[Yelle(2004)]{Yelle(2004)} Yelle, R.~V.\ 2004, \icarus, 170, 167 
